Multimodal Biometric Authentication Using Camera-Based PPG and Fingerprint Fusion

Camera-based photoplethysmography (PPG) obtained from smartphones has shown great promise for personalized healthcare and secure authentication. This paper presents a multimodal biometric system that integrates PPG signals extracted from videos with fingerprint data to enhance the accuracy of user verification. The system requires users to place their fingertip on the camera lens for a few seconds, allowing the capture and processing of unique biometric characteristics. Our approach employs a neural network with two structured state-space model (SSM) encoders to manage the distinct modalities. Fingerprint images are transformed into pixel sequences, and along with segmented PPG waveforms, they are input into the encoders. A cross-modal attention mechanism then extracts refined feature representations, and a distribution-oriented contrastive loss function aligns these features within a unified latent space. Experimental results demonstrate the system's superior performance across various evaluation metrics in both single-session and dual-session authentication scenarios.

==> refs.tex <==
@book{1,
  title={Handbook of fingerprint recognition},
  author={Maltoni, Davide and Maio, Dario and Jain, Anil K and Prabhakar, Salil and others},
  volume={2},
  year={2009},
  publisher={Springer}
}

@article{2,
  title={Touch-less palm print biometrics: Novel design and implementation},
  author={Michael, Goh Kah Ong and Connie, Tee and Teoh, Andrew Beng Jin},
  journal={Image Vis. Comput.},
  volume={26},
  number={12},
  pages={1551--1560},
  year={2008},
  publisher={Elsevier}
}

@article{3,
  title={Privacy--enhancing face biometrics: A comprehensive survey},
  author={Meden, Bla{\v{z}} and Rot, Peter and Terh{\"o}rst, Philipp and Damer, Naser and Kuijper, Arjan and Scheirer, Walter J and Ross, Arun and Peer, Peter and {\v{S}}truc, Vitomir},
  journal={IEEE Trans. Inf. Forensics Security},
  volume={16},
  pages={4147--4183},
  year={2021},
  publisher={IEEE}
}

@article{4,
  title={Recognition of human iris patterns for biometric identification},
  author={Ali, EM and Ahmed, ES and Ali, AF},
  journal={J. Eng. Appl. Sci. - Cairo},
  volume={54},
  number={6},
  pages={635},
  year={2007},
  publisher={FACULTY OF ENGINEERING CAIRO UNIVERSITY}
}

@article{5,
  title={Joint speaker verification and antispoofing in the $ i $-vector space},
  author={Sizov, Aleksandr and Khoury, Elie and Kinnunen, Tomi and Wu, Zhizheng and Marcel, S{\'e}bastien},
  journal={IEEE Trans. Inf. Forensics Security},
  volume={10},
  number={4},
  pages={821--832},
  year={2015},
  publisher={IEEE}
}

@article{6,
  title={Cardiovascular biometrics: combining mechanical and electrical signals},
  author={Odinaka, Ikenna and O’Sullivan, Joseph A and Sirevaag, Erik J and Rohrbaugh, John W},
 journal={IEEE Trans. Inf. Forensics Security},
  volume={10},
  number={1},
  pages={16--27},
  year={2014},
  publisher={IEEE}
}

@article{7,
  title={ECG biometric with abnormal cardiac conditions in remote monitoring system},
  author={Sidek, Khairul A and Khalil, Ibrahim and Jelinek, Herbert F},
  journal={IEEE Trans. Syst. Man Cybern. Syst.},
  volume={44},
  number={11},
  pages={1498--1509},
  year={2014},
  publisher={IEEE}
}

@article{8,
  title={Unveiling the biometric potential of finger-based ECG signals},
  author={Louren{\c{c}}o, Andr{\'e} and Silva, Hugo and Fred, Ana},
  journal={Comput. Intell. Neurosci.},
  volume={2011},
  pages={1--8},
  year={2011},
  publisher={Hindawi Limited London, UK, United Kingdom}
}

@inproceedings{9,
  title={A novel biometric approach in human verification by photoplethysmographic signals},
  author={Gu, YY and Zhang, Y and Zhang, YT},
  booktitle={Proc. 4th Int. IEEE EMBS Special Topic Conf. Inf. Technol. Appl. Biomed.},
  pages={13--14},
  year={2003}
}

@article{10,
  title={Evaluation of the time stability and uniqueness in PPG-based biometric system},
  author={Hwang, Dae Yon and Taha, Bilal and Lee, Da Saem and Hatzinakos, Dimitrios},
  journal={IEEE Trans. Inf. Forensics Security},
  volume={16},
  pages={116--130},
  year={2020},
  publisher={IEEE}
}

@inproceedings{11,
  title={Photoplethysmographic authentication through fuzzy logic},
  author={Gu, YY and Zhang, YT},
  booktitle={Proc. IEEE EMBS Asian–Pacific Conf. Biomed. Eng.},
  pages={136--137},
  year={2003}
}

@inproceedings{12,
  title={A pilot study on using derivatives of photoplethysmographic signals as a biometric identifier},
  author={Yao, Jianchu and Sun, Xiaodong and Wan, Yongbo},
  booktitle={Proc. 29th Annu. Int. Conf. IEEE Eng. Med. Biol. Soc.},
  pages={4576--4579},
  year={2007}
}

@inproceedings{13,
  title={Enhancement in the design of Biometric Identification System based on Photoplethysmography data},
  author={NS, Girish Rao Salanke and Sadhasivam, Dr Maheswari N S and Samraj, Dr Andrews},
  booktitle={Proc. Int. Conf. Green High Perform. Comput.},
  year={2013}
}

@inproceedings{14,
  title={Human recognition from photoplethysmography (ppg) based on non-fiducial features},
  author={Karimian, Nima and Guo, Zimu and Tehranipoor, Mark and Forte, Domenic},
  booktitle={ IEEE Int. Conf. Acoust. Speech Signal Process.(ICASSP)},
  pages={4636--4640},
  year={2017}
}

@inproceedings{15,
  title={An adaptive deep learning approach for PPG-based identification},
  author={Jindal, Vasu and Birjandtalab, Javad and Pouyan, M Baran and Nourani, Mehrdad},
  booktitle={Proc. 38th Annu. Int. Conf. IEEE Eng. Med. Biol. Soc. (EMBC)},
  pages={6401--6404},
  year={2016}
}

@inproceedings{16,
  title={A multimodal biometric identification system based on ECG and PPG signals},
  author={Yaacoubi, Chayma and Besrour, Rym and Lachiri, Zied},
  booktitle={Proc. 2nd Int. Conf. Digital Tools \& Uses Congress},
  pages={1--6},
  year={2020}
}

@article{17,
  author={Biswas, Dwaipayan and Everson, Luke and Liu, Muqing and Panwar, Madhuri and Verhoef, Bram-Ernst and Patki, Shrishail and Kim, Chris H and Acharyya, Amit and Van Hoof, Chris and Konijnenburg, Mario and others},
  title={CorNET: Deep learning framework for PPG-based heart rate estimation and biometric identification in ambulant environment},
  journal={IEEE Trans. Biomed. Circuits Syst.},
  volume={13},
  number={2},
  pages={282--291},
  year={2019},
  publisher={IEEE}
}

@ARTICLE{18,
  author={Chang, Hua-Chien and Wang, Ting and Liao, Chi-An and Liu, Tsung-Te},
  journal={IEEE Trans. Circuits Syst. II: Exp. Briefs}, 
  title={A Low-Power PPG Processor for Real-Time Biometric Identification and Heart Rate Estimation}, 
  year={2023},
  volume={70},
  number={10},
  pages={3932-3936},
  keywords={Estimation;Heart rate;Feature extraction;Hardware;Artificial neural networks;Frequency-domain analysis;Computational modeling;Low power;biometric identification;heart rate estimation;neural network (NN);photoplethysmography (PPG)},
  doi={10.1109/TCSII.2023.3291891}}

@inproceedings{19,
  title={Seeing red: PPG biometrics using smartphone cameras},
  author={Lovisotto, Giulio and Turner, Henry and Eberz, Simon and Martinovic, Ivan},
  booktitle={Proc. IEEE/CVF Conf. Comput. Vis. Pattern Recognit. Workshops},
  pages={818--819},
  year={2020}
}

@article{20,
  title={Efficiently modeling long sequences with structured state spaces},
  author={Gu, Albert and Goel, Karan and R{\'e}, Christopher},
  journal={arXiv preprint arXiv:2111.00396},
  year={2021}
}
  
@article{21,
  title={On the parameterization and initialization of diagonal state space models},
  author={Gu, Albert and Goel, Karan and Gupta, Ankit and R{\'e}, Christopher},
  journal={Adv. Neural Inf. Process. Syst.},
  volume={35},
  pages={35971--35983},
  year={2022}
}

@INPROCEEDINGS{22,
  author={Pizer, S.M. and Johnston, R.E. and Ericksen, J.P. and Yankaskas, B.C. and Muller, K.E.},
  booktitle={Proc. First Conf. Vis. Biomed. Comput.}, 
  title={Contrast-limited adaptive histogram equalization: speed and effectiveness}, 
  year={1990},
  volume={},
  number={},
  pages={337-345},
  keywords={Histograms;Adaptive equalizers;Biomedical imaging;Computed tomography;Displays;Lesions;Lungs;Clinical diagnosis;Design methodology;Medical diagnostic imaging},
  doi={10.1109/VBC.1990.109340}}

@article{23,
  title={Canny edge detection enhancement by scale multiplication},
  author={Bao, Paul and Zhang, Lei and Wu, Xiaolin},
  journal={IEEE Trans. Pattern Anal. Mach. Intell.},
  volume={27},
  number={9},
  pages={1485--1490},
  year={2005},
  publisher={IEEE}
}


@article{24,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Adv. Neural Inf. Process. Syst.},
  volume={30},
  year={2017}
}

@article{25,
  title={Representation learning with contrastive predictive coding},
  author={Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1807.03748},
  year={2018}
}

@inproceedings{26,
  title={Delving into deep imbalanced regression},
  author={Yang, Yuzhe and Zha, Kaiwen and Chen, Yingcong and Wang, Hao and Katabi, Dina},
  booktitle={Proc. Int. Conf. Mach. Learn. (ICML)},
  pages={11842--11851},
  year={2021},
  organization={PMLR}
}

@inproceedings{27,
  title={Non-fiducial ppg-based authentication for healthcare application},
  author={Karimian, Nima and Tehranipoor, Mark and Forte, Domenic},
  booktitle={Proc. IEEE EMBS Int. Conf. Biomed. Health Informat. (BHI)},
  pages={429--432},
  year={2017}
}

@article{28,
  title={Biometric authentication using the PPG: A long-term feasibility study},
  author={Sancho, Jorge and Alesanco, {\'A}lvaro and Garc{\'\i}a, Jos{\'e}},
  journal={Sensors},
  volume={18},
  number={5},
  pages={1525},
  year={2018}
}

@inproceedings{29,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proc. IEEE Conf. Comput. Vis. Pattern Recognit.},
  pages={770--778},
  year={2016}
}


%%%
@article{hwang2021pbgan,
  title={PBGAN: Learning PPG representations from GAN for time-stable and unique verification system},
  author={Hwang, Dae Yon and Taha, Bilal and Hatzinakos, Dimitrios},
  journal={IEEE Trans. Inf. Forensics Security},
  volume={16},
  pages={5124--5137},
  year={2021},
  publisher={IEEE}
}

@inproceedings{hwang2021variation,
  title={Variation-stable fusion for PPG-based biometric system},
  author={Hwang, Dae Yon and Taha, Bilal and Hatzinakos, Dimitrios},
  booktitle={IEEE Int. Conf. Acoust. Speech Signal Process.(ICASSP)},
  pages={8042--8046},
  year={2021},
  organization={IEEE}
}

@article{hwang2022new,
  title={A new score level fusion approach for stable user verification system using the PPG signal},
  author={Hwang, Dae Yon and Taha, Bilal and Hatzinakos, Dimitrios},
  journal={J. Signal Process. Syst.},
  volume={94},
  number={8},
  pages={787--798},
  year={2022},
  publisher={Springer}
}

@article{siam2021biosignal,
  title={Biosignal classification for human identification based on convolutional neural networks},
  author={Siam, Ali I and Sedik, Ahmed and El-Shafai, Walid and Elazm, Atef Abou and El-Bahnasawy, Nirmeen A and El Banby, Ghada M and Khalaf, Ashraf AM and Abd El-Samie, Fathi E},
  journal={International journal of communication systems},
  volume={34},
  number={7},
  pages={e4685},
  year={2021},
  publisher={Wiley Online Library}
}
